Transferable Deep Clustering Model

Deep learning has shown remarkable success in the field of clustering recently. However, how to transfer a trained clustering model on a source domain to a target domain by leveraging the acquired knowledge to guide the clustering process remains challenging. Existing deep clustering methods often lack generalizability to new domains because they typically learn a group of fixed cluster centroids, which may not be optimal for the new domain distributions. In this paper, we propose a novel transferable deep clustering model that can automatically adapt the cluster centroids according to the distribution of data samples. Rather than learning a fixed set of centroids, our approach introduces a novel attention-based module that can adapt the centroids by measuring their relationship with samples. In addition, we theoretically show that our model is strictly more powerful than some classical clustering algorithms such as k-means or Gaussian Mixture Model (GMM). Experimental results on both synthetic and real-world datasets demonstrate the effectiveness and efficiency of our proposed transfer learning framework, which significantly improves the performance on target domain and reduces the computational cost.

==> old_method.tex <==
Therefore, we modify the score function $\delta_{ij}^{(l+1)}$ in Equation~\ref{eq:iterative} to an attention-like manner:
\begin{equation}\label{eq:attention} 
\begin{split}
    \delta_{ij}^{(l+1)} & = \frac{\exp{( \sigma (\mathbf{W}_Q\mathbf{z}_i \cdot \mathbf{W}_K \mathbf{c}_j^{(l)})/\tau)}}{\sum_{j=1}^{K}{\exp{(- \sigma (\mathbf{W}_Q\mathbf{z}_i \cdot \mathbf{W}_K \mathbf{c}_j^{(l)})/\tau)}}}, 
\end{split}
\end{equation}
where $\mathbf{W}_Q$ and $\mathbf{W}_K$ are two learnable matrices and $\sigma$ is a nonlinear activation function.


Unfortunately, simply adopting the above commonly used attention based score function can not guarantee the similarity relationship between samples can be correclty revealed by the learned score function, which may leads to the failure of capturing the true pattern of clusters. 


 as:
\begin{equation}
\begin{split}
    \mathcal{L}_{\mathrm{clustering}} &= -\sum_l^{L} \alpha^{(l)} \sum_i^{N} \sum_j^{K} \delta_{ij}^{(l)} \ell(\mathbf{z}_i, \mathbf{c}_j^{(l)}) + \lambda(\|\mathbf{W}_Q  \mathbf{W}_Q^\intercal - \mathbf{I}\|_2^2+\|\mathbf{W}_K  \mathbf{W}_K^\intercal - \mathbf{I}\|_2^2)
\end{split}
\end{equation}
where $\lambda$ is a hyperparameter controlling the importance of the regularization term. 
